Stability of the nonlinear filter for slowly switching Markov chains

Exponential stability of the nonlinear filtering equation is revisited, when the signal is a finite state Markov chain. An asymptotic upper bound for the filtering error due to incorrect initial condition is derived in the case of slowly switching signal.

==> scl/another-version/gammaeps.tex <==
\pspicture(0,0)(9,-4)
\psaxes*[linewidth=1.2pt,labels=all,ticks=all,ticksize=0.02,tickstyle=full,Dx=0.05,dx=1,Dy=0.25,dy=1]{<->}(0,0)(0,-4)(4,0)
\fileplot{gamma-list.dat}
\rput(4.2,0.0){$\lambda$}
\rput(-0.5,-3.8){$\gamma(\lambda)$}
\rput(2.0,-3.5){Wonham}
%\psline[linewidth=0.2pt, linestyle=dashed]{-}(0.5,0)(0.5,-1.8)
%\psbezier[linewidth=0.5pt,showpoints=true]{->}(2.0,-1.0)(1.5,-2.5)(1.0,-1.0)(0.5,-1.8)

\psaxes*[linewidth=1.2pt,labels=all,ticks=all,ticksize=0.02,tickstyle=full,Dx=0.05,dx=1,Dy=0.25,dy=1]{<->}(6,0)(6,-4)(10,0)
\rput(6,0){\psplot[plotpoints=100]{0}{4}{0.0 0.05 x mul 0.05 x mul mul 0.05 x mul 2 mul add sqrt sub 4 mul}}
\rput(10.2,0.0){$\lambda$}
\rput(5.5,-3.8){$\gamma(\lambda)$}
\rput(8.0,-3.5){Kalman-Bucy}
\endpspicture


==> spa/gammaeps.tex <==
\pspicture(-1.0,-4.5)(4.0,1.0)
\psaxes*[linewidth=0.5pt,ticks=none,labels=none]{->}(0,0)(0,-4)(3,0.5)
\rput(3.3,0){\footnotesize $\eps$} \rput(-0.25,0){\footnotesize
$0$} \psdots*[dotstyle=o,dotsize=2.0pt](0,-1.5)
\psdots*[dotstyle=*,dotsize=2.0pt](0,0)
\pscurve[linewidth=0.5pt]{->}(0,-1.5)(1.0,-0.5)(2.4,-4)
\psline[linewidth=0.5pt,linestyle=dotted,dotsep=1.5pt](2.5,0)(2.5,-4)
\rput(2.3,-4.2){\footnotesize $-\infty$}
\psdots*[dotstyle=*,dotsize=2.0pt](2.5,0)
\rput(2.5,0.3){\footnotesize $\frac{1}{2\lambda}$}
\psline[linewidth=0.5pt,linestyle=dotted,dotsep=1.5pt](0.95,0.0)(0.95,-0.5)
\rput(1.0,0.2){\footnotesize $\eps^\star$}
\rput(-0.55,-1.5){\footnotesize $-\D_p$}
\psline[linewidth=0.5pt,linestyle=dotted,dotsep=1.5pt](0.0,-1.5)(0.55,-1.5)
\psline[linewidth=0.5pt,linestyle=dotted,dotsep=1.5pt]{<->}(0.4,-0.9)(0.4,-1.5)
\psline[linewidth=0.5pt,linestyle=dotted,dotsep=1.5pt](0.4,-1.5)(0.4,-2.0)
%\psbezier[linewidth=0.1pt,showpoints=false]{<-}(0.15,-1.3)(1.0,-1.5)(0.5,-1.8)(1.0,-2.0)
\rput(1.0,-2.1){\footnotesize $\sim \eps\log\frac{1}{\eps}$}
\rput(0,0.7){\footnotesize $\gamma(\eps)$}
\endpspicture

